Optimizing Communication by Compression for Multi-GPU Scalable Breadth-First Searches

The Breadth First Search (BFS) algorithm is the foundation and building block of many higher graph-based operations such as spanning trees, shortest paths and betweenness centrality. The importance of this algorithm increases each day due to it is a key requirement for many data structures which are becoming popular nowadays. When the BFS algorithm is parallelized by distributing the graph between several processors the interconnection network limits the performance. Hence, improvements on this area may benefit the overall performance of the algorithm. This work presents an alternative compression scheme for communications in distributed BFS processing. It focuses on BFS processors using General-Purpose Graphics Processing Units.

==> titlepages-ger.tex <==
%% Titelseiten ähnlich zum Layout des Formulars von der
%% Fakultät für Physik und Astronomie
%%
%% Weitere Infos:
%% http://www.physik.uni-heidelberg.de/aktuelles/studium/
%% (PDF link: ...studium/download/145/Vorlage_Diplomarbeit_Formular.pdf)

%% Titelintro
\thispagestyle{empty}
\begin{center}
  \renewcommand{\baselinestretch}{2.00}
  \Large\sffamily
  Fakult\"{a}t f\"{u}r Physik und Astronomie\\
  \large
  Ruprecht-Karls-Universit\"{a}t Heidelberg
  \par\vfill\normalfont
  Masterarbeit\\
  Im Studiengang Physik\\
  vorgelegt von\\
  (Vor- und Zuname)\\
  geboren in (Geburtsort)\\
  (Jahr der Abgabe)\\
\end{center}
\newpage

%% Titelseite
\thispagestyle{empty}
\begin{center}
  \renewcommand{\baselinestretch}{2.00}
  \Large\bfseries\sffamily
    (Titel)\\
    (der)\\
    (Masterarbeit)
  \par
  \vfill
  \large\normalfont
  Die Masterarbeit wurde von (Vorname Name)\\
  ausgef\"{u}hrt am\\
  (Institut)\\
  unter der Betreuung von\\
  (Frau/Herrn Prof./Priv.-Doz. Vorname Name)
  %% Bei externen Masterarbeiten hier noch den zweiten Betreuer einfügen
  %% und den vspace in Z. 45 entsprechend reduzieren
\end{center}\par
\vspace{5\baselineskip}

% Zeilenabstand zurücksetzen
\renewcommand{\baselinestretch}{1.00}\normalsize
